GPU-accelerated partially linear multiuser detection for 5G and beyond URLLC systems

In this feasibility study, we have implemented a recently proposed partially linear multiuser detection algorithm in reproducing kernel Hilbert spaces (RKHSs) on a GPU-accelerated platform. Partially linear multiuser detection, which combines the robustness of linear detection with the power of nonlinear methods, has been proposed for a massive connectivity scenario with the non-orthogonal multiple access (NOMA). This is a promising approach, but detecting payloads within a received orthogonal frequency division multiplexing (OFDM) radio frame requires the execution of a large number of inner product operations, which are the main computational burden of the algorithm. Although inner-product operations consist of simple kernel evaluations, their vast number poses a challenge in ultra-low latency (ULL) applications, because the time needed for computing the inner products might exceed the sub-millisecond latency requirement. To address this problem, this study demonstrates the acceleration of the inner-product operations through massive parallelization. The result is a GPU-accelerated real-time OFDM receiver that enables sub-millisecond latency detection to meet the requirements of 5th generation (5G) and beyond ultra-reliable and low latency communications (URLLC) systems. Moreover, the parallelization and acceleration techniques explored and demonstrated in this study can be extended to many other signal processing algorithms in Hilbert spaces, such as those based on projection onto convex sets (POCS) and adaptive projected subgradient method (APSM) algorithms. Experimental results and comparisons with the state-of-art confirm the effectiveness of our techniques.

==> sections/biographies.tex <==
% magic comments for TeXworks
% ------------------------------------------------------------------------------
% !TeX program = pdfLaTeX+MakeIndex+BibTeX
% !TeX encoding = UTF-8
% !TeX spellcheck = en_US
% !TeX root = ../2022_noma_cuda_demonstrator_IEEEaccess.tex
% ------------------------------------------------------------------------------

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% break the column
\newpage
\phantomsection %\label{biographies}
\addcontentsline{toc}{section}{Biographies}
%\section*{Biographies}

%
% Matthias
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace*{-2\baselineskip}
%\begin{IEEEbiography}[{\includegraphics[viewport=485 0 1533 1310, width=1in, height=1.25in, clip, keepaspectratio]{authors/a1}}]{\PAPERauthorOne}
\begin{IEEEbiography}[{\includegraphics[viewport=675 450 1235 1150, width=1in, height=1.25in, clip, keepaspectratio]{authors/a1}}]{\PAPERauthorOne}
%has an educational background as a communication electronics technician.
received his \mbox{Dipl.-Ing.~(FH)} graduation in telecommunications and communications techniques from the University of Applied Sciences for Engineering and Economics (FHTW) Berlin in 2008 and a Master of Science degree in electrical engineering from the Technical~University of Berlin (TU Berlin) in 2011.
He started his employment at Fraunhofer Institute for Telecommunications, Heinrich Hertz Institute (HHI), in the Wireless Communications and Networks department in 2007 with an internship.
Until 2012 he works there as a student assistant.
Since then, he has been working as a research associate and engineer.

His research interest address the implementation of real-time signal processing algorithms on multi-core processors with high-speed data links to \ac{SDR} systems equipped with massive \ac{MIMO} antenna arrays.
\end{IEEEbiography}
\vspace*{-1\baselineskip}
%
% break the column
%\vfill
%\newpage
%
% Guillermo
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-2\baselineskip}
\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in, clip, keepaspectratio]{authors/a4}}]{\PAPERauthorFour}
is a senior software engineer at NVIDIA at the intersection of graphics, communications, and machine learning. He is interested in software engineering and applied scientific computing with a focus on accelerated computing and application-specific accelerators. He received the PRACE Award at ISC 2011, and joined NVIDIA in 2013. He has a Ph.D. (magna cum laude) from the Heidelberg University in Germany, a M.Sc. from Instituto Tecnológico y de Estudios Superiores de Monterrey in Mexico, and an Electronics Engineering degree from Simón Bolívar University in Venezuela.
\end{IEEEbiography}
\vspace*{-1\baselineskip}
%
% break the column
%\vfill
%\newpage
%
% Daniel
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-2\baselineskip}
\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in, clip, keepaspectratio]{authors/a2}}]{\PAPERauthorTwo}
received the B.Sc. degree in IT-Systems engineering from the Hasso-Plattner-Institute, University of Potsdam, Germany, in 2012 and the B.Sc. and M.Sc. degrees in computer engineering from Technical University of Berlin, Germany in 2015 and 2017, respectively.

He is currently a research associate with the Fraunhofer Institute for Telecommunications, Heinrich Hertz Institute, Berlin, Germany. His  interests are applying machine learning algorithms to wireless communication systems.
\end{IEEEbiography}
\vspace*{-1\baselineskip}
%
% break the column
%\vfill
%\newpage
%
% Daniyal
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-2\baselineskip}
\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in, clip, keepaspectratio]{authors/a3}}]{\PAPERauthorThree}
received the M.Sc. and Ph.D. (\textit{summa cum laude}) degrees in electrical engineering from the Technical University of Berlin (TU Berlin), Germany, in 2013 and 2020, respectively.
He is currently a research associate with the Fraunhofer Institute for Telecommunications, Heinrich Hertz Institute (HHI), Berlin, Germany.
Previously, he worked as a Research Associate at the TU Berlin and as a Guest Researcher at the HHI.
His research revolves around application of optimization theory, function analysis, and machine learning to problems in wireless communication systems.
\end{IEEEbiography}
\vspace*{-1\baselineskip}
%
% break the column
%\vfill
%\newpage
%
% Nikolaus
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-2\baselineskip}
\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in, clip, keepaspectratio]{authors/a5}}]{\PAPERauthorFive}
is a senior research scientist at NVIDIA.
He joined NVIDIA in 2011.
Before he received his MS degree in computer science from the University of Ulm, Germany, helped planning and implementing several government funded projects for two companies, maintained their IT infrastructure, and worked for the mental images GmbH as a research consultant.

His research, publications, and presentations are focused on quasi-Monte Carlo methods, photorealistic image synthesis, ray tracing, and rending algorithms with a strong emphasis on the underlying mathematical and algorithmic structure.
\end{IEEEbiography}
\vspace*{-1\baselineskip}
%
% break the column
%\vfill
\newpage
%
% Martin
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace*{-2\baselineskip}
\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in, clip, keepaspectratio]{authors/a6}}]{\PAPERauthorSix}
received the Dipl.-Ing. degree and the Dr.-Ing. degree from the Technische Universit\"at Berlin (TU Berlin), Germany, in 2009 and 2015, respectively. From 2010 to 2013, he had been a research associate with the Heinrich Hertz Chair of Information Theory and Theoretical Information Technology, TU Berlin. Since 2013, he has been with the Fraunhofer Institute for Telecommunications, Heinrich Hertz Institute (HHI), Berlin. Currently, he leads the Signal and Information Processing Group at the Fraunhofer HHI. His current interests are in the area of network optimization, V2X communications, software defined radio, and the application of machine learning to wireless communication systems. 
\end{IEEEbiography}
\vspace*{-1\baselineskip}
%
% break the column
%\vfill
%\newpage
%
% Renato
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-2\baselineskip}
\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in, clip, keepaspectratio]{authors/a7}}]{\PAPERauthorSeven}
(M’09) received the Electronics Engineering degree from the Instituto Tecnológico de Aeronáutica, São José dos Campos, Brazil, in 2002, and the M.E. and Ph.D. degrees in communications and integrated systems from the Tokyo Institute of Technology, Tokyo, Japan, in 2006 and 2008, respectively. 
He  is  currently  a  Research  Fellow  with the Fraunhofer Institute for Telecommunications, Heinrich Hertz Institute (HHI), Berlin, Germany, and a lecturer with the Technical University of Berlin. Previously, he held appointments as a research fellow with the University of Southampton, U.K., and as a research Associate with the University of Edinburgh, U.K. 
His current interests include signal processing for distributed systems, multiagent systems, convex analysis, machine learning, and wireless communications. Dr. Cavalcante received the Excellent Paper Award from the Institute of Electronics, Information and Communication Engineers in 2006 and the IEEE Signal Processing Society (Japan Chapter) Student Paper Award in 2008. He also co-authored a study that received a Best Student Paper Award at the 13th IEEE International Workshop on Signal Processing Advances in Wireless Communications in 2012. From April 2003 to April 2008, he was a recipient of the Japanese Government (MEXT) Scholarship.
\end{IEEEbiography}
\vspace*{-1\baselineskip}
%
% break the column
%\vfill
%\newpage
%
% Slawomir
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-2\baselineskip}
\begin{IEEEbiography}[{\includegraphics[viewport=340 0 1020 850, width=1in, height=1.25in, clip, keepaspectratio]{authors/a8}}]{\PAPERauthorEight}
% Prof. Dr.-Ing. habil. Slawomir Stanczak
% slawomir.stanczak@tu-berlin.de
% slawomir.stanczak@hhi.fraunhofer.de
% Phone +49 30 31002 875
% short version
%\comment{
\comment{S\lawomir Sta\'nczak} studied electrical engineering with specialization in control theory at the Wroclaw University of Technology and at the Technical University of Berlin (TU Berlin).
He received the Dipl.-Ing. degree in 1998 and the Dr.-Ing. degree (summa cum laude) in electrical engineering in 2003, both from the TU Berlin; the habilitation degree (venialegendi) followed in 2006.
Since 2015, he has been a full professor for network information theory with the TU Berlin and the head of the Wireless Communications and Networks department at Fraunhofer Institute for Telecommunications, Heinrich Hertz Institute (HHI).
Prof. Sta\'nczak is a co-author of two books and more than 200 peer-reviewed journal articles and conference papers in the area of information theory, wireless communications, signal processing and machine learning.
He was an Associate Editor of the IEEE Transactions on Signal Processing between 2012 and 2015.
From February 2018 to July 2020 Prof. Sta\'nczak was the chairman of the ITU-T focus group on machine learning for future networks including 5G.
%}
% long version
\comment{
\comment{S\lawomir Sta\'nczak} studied electrical engineering with specialization in control theory at the Wroc{\l}aw University of Technology and at the Technical University of Berlin (TU Berlin).
He received the Dipl.-Ing. degree in 1998 and the Dr.-Ing. degree (summa cum laude) in electrical engineering in 2003, both from TU Berlin; the Habilitation degree (venialegendi) followed in 2006.
Since 2015, he has been a Full Professor for network information theory with the TU Berlin and the head of the Wireless Communications and Networks department at Fraunhofer Institute for Telecommunications, Heinrich Hertz Institute (HHI).
Prof. Sta\'nczak has been involved in research and development activities in wireless communications since 1997. In 2004 and 2007, he was a Visiting Professor with RWTH Aachen University and in 2008, he was a Visiting Scientist with Stanford University, Stanford, CA, USA.
He is a co-author of two books and more than 200 peer-reviewed journal articles and conference papers in the area of information theory, wireless communications, signal processing and machine learning.
Prof. Sta\'nczak received research fellowships from the German Research Foundation and the Best Paper Award from the German Communication Engineering Society in 2014.
He was a Co-chair of the 14th International Workshop on Signal Processing Advances in Wireless Communications (SPAWC 2013).
Between 2009 and 2011, he was an Associate Editor of the European Transactions for Telecommunications (information theory) and an Associate Editor of the IEEE Transactions on Signal Processing between 2012 and 2015.
From February 2018 to July 2020 Prof. Sta\'nczak was the chairman of the ITU-T focus group on machine learning for future networks including 5G.
}
\end{IEEEbiography}
\vspace*{-1\baselineskip}
%
% break the column
%\vfill
%\newpage
%
% Alex
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace*{-2\baselineskip}
\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in, clip, keepaspectratio]{authors/a9}}]{\PAPERauthorNine}
is a Director of Research at NVIDIA.
Before, he had been the Chief Scientist of mental images.
Prior to industry, he worked as a full professor for computer graphics and scientific computing at Ulm University.
He holds a Dr. rer. nat. degree (summa cum laude) from the Technical University of Kaisers\-lautern.

Alexander Keller has more than 3 decades of experience in ray tracing, pioneered quasi-Monte Carlo methods for light transport simulation that are used across industries, and connected the domains of machine learning and transport simulation.
His research interests include wireless communication systems, machine learning, and computer graphics.
\end{IEEEbiography}
\vspace*{-1\baselineskip}
%
% break the column
%\vfill
%\newpage

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

